"Understanding Robustness Lottery": A Geometric Visual Comparative Analysis of Neural Network Pruning Approaches

Deep learning approaches have provided state-of-the-art performance in many applications by relying on large and overparameterized neural networks. However, such networks have been shown to be very brittle and are difficult to deploy on resource-limited platforms. Model pruning, i.e., reducing the size of the network, is a widely adopted strategy that can lead to a more robust and compact model. Many heuristics exist for model pruning, but empirical studies show that some heuristics improve performance whereas others can make models more brittle or have other side effects. This work aims to shed light on how different pruning methods alter the network's internal feature representation and the corresponding impact on model performance. To facilitate a comprehensive comparison and characterization of the high-dimensional model feature space, we introduce a visual geometric analysis of feature representations. We decomposed and evaluated a set of critical geometric concepts from the common adopted classification loss, and used them to design a visualization system to compare and highlight the impact of pruning on model performance and feature representation. The proposed tool provides an environment for in-depth comparison of pruning methods and a comprehensive understanding of how model response to common data corruption. By leveraging the proposed visualization, machine learning researchers can reveal the similarities between pruning methods and redundant in robustness evaluation benchmarks, obtain geometric insights about the differences between pruned models that achieve superior robustness performance, and identify samples that are robust or fragile to model pruning and common data corruption to model pruning and data corruption but also obtain insights and explanations on how some pruned models achieve superior robustness performance.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Userstudy.tex <==
\section{User Study}
In this section, we will introduce the knowledge expertise of our participants in graph visualization; the statistic property of the dataset we use, and how we setup the experiment.

 % This is a replicate study of previous research~\cite{ghoniem2004comparison} with one additional matrix-link visual encoding in the experiment.

\subsection{Participants}
We did our user study with 9 participants. Each participant is a graduate student from the school of engineering at the University. Before the experiment, We asked them how much they are familiar with the graph visualization.  The metric value is range from 1 to 5. If the participant claim her/his expertise as 1, then he/she is not familiar graph visualization, and 5 means he/she is an expert. The expertise of the participants are summarize in Figure~\ref{fig:expertise_of_graph}. Two of them answer 3.5, two of them answered 3, four of them answered 2 and one person answers 1. Since some participants are not familiar with the graph visualization, we have to do a simple training section to teach each of them what they are looking at and how to perform the specific tasks.
    
\begin{figure}[t]
\centering
    \includegraphics[width=\linewidth]{image/10_1_Familiar.pdf}
    \vspace{-3mm}
    \caption{The expertise of participants in the graph visualization. 1 means not familiar with it. 5 means a expert in this area.}
    \label{fig:expertise_of_graph}
\end{figure}    
    
    
\subsection{Dataset}
The experiment have 10 graph datasets and each participant needs to view 10 datasets (15 nodes, 30 nodes, 50 nodes, and 100 nodes) with the 20\% network density for each visual encoding. Only one dataset has 15 nodes and it is used for teaching purpose. Each dataset is generate by a random graph generator with \textit{Networkx} python library. The length of the shortest path between two nodes in  each dataset is presented in Figure~\ref{fig:shorest_path_length_distribution}. The mean shortest path of graph with 30 nodes is 2.83, and the mean of the graph with 50 nodes is 2.82, and the mean of the graph with 100 nodes is 2.76. During the experiment, the computer randomly picked two nodes and asked the participant to find a path between two nodes.


\begin{figure*}
\centering
    \includegraphics[width=2.3in]{image/10_2_30_distribution.pdf}
    \includegraphics[width=2.3in]{image/10_2_50_distribution.pdf}
    \includegraphics[width=2.3in]{image/10_2_100_distribution.pdf}
    \caption{The shortest path length distribution between two nodes over each scale dataset. Most of nodes in each dataset can reach each other with 2 or 3 steps and a few of nodes need 4 or 5 steps.}
\label{fig:shorest_path_length_distribution}
\vspace{-4mm}
\end{figure*}


\subsection{Visual encoding}
In this user study, we compared users' performance on three different visual encoding;node-link diagram; adjacency matrix and matrix-link visualization. For node-link diagram, we use the standard graph-force layout. For the adjacency matrix and matrix-link, we use the optimal-leaf-order algorithm to order the element of the matrix before it presented to the participants. Due to the complexity of some graph tasks in large dataset (e.g. find-path tasks in dataset with 100 nodes), the visualization we present to the participant support highlight operation, which enable to highlight a node and paths that connected to this node.


\begin{figure*}
\centering
    \includegraphics[width=2.3in]{image/10_3_graph.png}
    \includegraphics[width=2.3in]{image/10_3_matrix.png}
    \includegraphics[width=2.3in]{image/10_3_matrixlink.png}
    \caption{The shortest path length distribution between two nodes over each dataset. Each visualization support basic highlight operation. Here are three different visualizations of 30 nodes dataset that we used in our user study.}
\label{fig:shorest_path_length_distribution}
\vspace{-4mm}
\end{figure*}

\subsection{User Study Tasks}
In this study, we perform four tasks to evaluate the performance of each visual encoding. Task 1 and 2 are basic graph exploration task. Task 3 and 4 are important for our domain experts. The node which has the most dependency (most-Connected) can have large impact on error propagation. Find a path between two nodes in the dependency graph will help to understand how error is propagated from one to the other.
\begin{itemize}
    \item Task 1: approximate estimation of the number of nodes in the graph, referred to as 'node-Count'. During the experiment, we will ask the participant "How many nodes in the visualization?".
    

    \item Task 2: finding a node given its label, referred to as 'find-Node'.  During the experiment, we will ask the participant "Can you find node X?"
    
    \item Task 3: finding the most connected node, referred to as 'most-Connected'.  During the experiment, we will ask the participant "which node has the most connection?".
    
    
    \item Task 4: finding a path between two nodes, referred to as “find-Path”.  During the experiment, we will ask the participant "Can you can a path between node X and node Y?"
\end{itemize}


\subsection{Experiment Setup and Process}
During the interview process, we placed the participant in a quiet meeting room without distraction. The visualization is presented in a 13 inch Mac book. The interview is performed in an interactive manner that we ask the participant a question with a timer and wait until he/she give us an answer to the question. We estimate the time to finish the task by calculate the time gap between we ask the question and the participant answer the questions.
For each tasks, we limit the participant to answers the question in 45 seconds. If the time pass 45 seconds, we will let the participant continue the research but mark the task as failure.
Each 

Our study can be formalized in following steps:
\begin{itemize}
    \item The experiment begin with a tutorial section. We use the dataset with 15 nodes as a tutorial dataset to teach each participant the meaning of each visualization and how the interaction in the visualization work. Each participant need to perform Task 1-4 in this dataset before they officially start the experiment.
    
    \item After the tutorial section, we started to record the performance of each participant on different dataset. The experiment start to evaluate one visualization with 30 nodes and perform Task 1 to 4. Once the participant done with the task, he/she will continue to the same visualization with 50 nodes and 100 nodes.
    
    \item Once the participant finish all the Tasks, we allow the participant to take a break for 5 minute. We will reconfigure the environment and configuration in the computer and continue experiment with the new visual encoding. The experiment will repeat this process until he/she finish all the tasks. 
\end{itemize}
The order that we present our visual encoding to different participant is different. We select the presentation order in  Matrix-Graph-Link, Link-Matrix-Graph, Graph-Link-Matrix, and repeat it.

\subsection{Experiment Result}
During the study, we record the time that each participant finishes each task and the correctness of their answers. We do statistic analysis on the record data and use the result to compare the performance of each visual encoding.




\subsection{Experiment Discussion}
Some participant will get familiar with the task and can perform task faster event in new visual encoding. We present our visualization on the visualization browser environment and the participant will randomly click with mouse and sometime this will cause browser link to something complete unrelated to this research.

==> backup.tex <==




\subsection{How do pruning and retrain schemes impact network latent representations?}
The previous use case demonstrates that some model architectures and pruning approaches have better performance than others. However, what in the geometry of latent space causes such a difference?
Here, we demonstrate how a model's latent space is impacted by the pruning operation, and compare different pruning approaches in terms of their impact on the latent representation of clean test data.
Model pruning is often evaluated with prediction accuracy on clean test data but with limited information about their impact on a model's internal representation, i.e, latent spaces, which may help shed light on their true capability.

\begin{figure*}[t]
\centering
    \includegraphics[width=\linewidth]{images/7_use_case_6.pdf}

    \vspace{-3mm}
    \caption{Compared with the pre-trained model, magnitude pruning with $50\%$, $70\%$, and $90\%$ pruning ratio will decrease the geometric features margin, \emph{length}, and increase the \emph{angle}. Comparing the pre-trained model with pruning and retraining, the retrain operation increases \emph{length} and \emph{margin} dramatically. However, \emph{angle} will decrease with the increasing pruning ratio. \textcolor{red}{can you make this use case generalize.}}
\label{fig:use_case_7_6}
\vspace{-4mm}
\end{figure*}

In Fig.~\ref{fig:use_case_7_1}, the original model is a VGG16 that trained on the cifar10 dataset.
After training, the accuracy of the final model is 91\%.
Here we show samples from the plane class, and their \emph{angle} with respect to each class direction is displayed in Fig.~\ref{fig:use_case_7_1} \textcircled{\small{1}}. We can see that the initial dense (or unpruned) model may confuse the plane samples with the bird and ship samples.

With the first-order Taylor pruning, the accuracy of the model drops to 77\% and the pruned model (Fig.~\ref{fig:use_case_7_1} \textcircled{\small{2}}) increases the chance of confusing the plane samples with the bird samples.
The probability that plane samples are confused with ship samples slightly decreases, whereas the chance of confusing them with truck samples and deer samples increases. 


For random pruning, only 10\% of weights  removed from the model can significantly damage the performance of the model. 
The operation decreases the model's (Fig.~\ref{fig:use_case_7_1} \textcircled{\small{3}}) performance to 73\%, and changes the plane samples' \emph{angles} dramatically such that they become closer to the cat's class direction. 
However, the ambiguity between the plane class and cat class is not the main concern in the dense well-trained model and the model generated by other pruning approaches.


The magnitude pruning generates a model (Fig.~\ref{fig:use_case_7_1} \textcircled{\small{4}}) with a comparable 79\% accuracy through removing 70\% of the weights. However, the resulting model amplifies the ambiguity of the plane samples with the bird and ship samples.
The uncertainty between the plane and frog samples also increases.


%The next model (Fig.~\ref{fig:use_case_7_1}\textcircled{\small{5}}) is the retrained model after pruning 99\% weights of a model, and retraining the model with the original data to recover the loss in accuracy.
%The \emph{angle} of plane class samples does not completely recover along the plane class direction, and the ambiguity among plane, bird and ship samples still exist in the the new representation. 


The last model (Fig.~\ref{fig:use_case_7_1} \textcircled{\small{5}}) uses the untrained VGG16 model pruned with MPTs. 
The \emph{angle} of the plane samples is relatively small compared to other class directions. 
Meanwhile, these samples' \emph{angle} with other class directions is close to 90 degrees, and they have a much small standard deviation compared to other models. This result is rather surprising for domain experts, as it shows that \emph{MPT pruning can be used to refine the model geometry as opposed to the popular belief that pruning only maintains or hurts the original model's behavior~\cite{hooker2019compressed}.
Meanwhile, domain experts also think that the observation in Fig.~\ref{fig:use_case_7_1} also inspired them to use the presented visualization 
to assemble multiple pruned models to design a compact model that is more robust and accurate based on their geometric features, which is part of the future work.}

From the above comparison, we can tell why one model pruning method behaves better than the other on certain subset samples, but what causes a pruned model to perform better than a pretrain model.
In Fig.~\ref{fig:use_case_7_6}, we can tell from the pre-trained and pruning sections that pruning will increase angle and decrease margin and l2 norm.
However, if the pruning ratio does not exceed a certain threshold, then the angle can still be recovered.
In Fig.~\ref{fig:use_case_7_6} right, we can tell that with $50\%$ weight pruned and retrained, the angle of feature representation is recovered. 
The l2 norm and margin value distribution exceed the original distribution and become much larger. 
With $70\%$ and $90\%$ weight pruned, the angle distribution does not recover to the original distribution but the l2 norm and margin are still larger than the pretrained model.
All retrained models still have better performance than the pretrain model.
We also check the feature attribution heat map with respect to the margin in Fig.~\ref{fig:use_case_7_2_2}. 
We compare the geometric feature attribution heat map of the pretrained model and retrained model with $50\%$ weight pruned.
We select Fig.~\ref{fig:use_case_7_2_2}(\textcircled{\small{1}}) samples (green color) that are predicted incorrectly in the pre-train model but correctly in the retrained model.
The geometric feature attribution visualization in Fig.~\ref{fig:use_case_7_2_2}(\textcircled{\small{3}}) shows that the retrained model captures better features than the pretrain model.



%Model pruning affects different samples in different ways.
%By comparing two VGG16 models with the same performance accuracy but one of them is pruned 50\% with magnitude pruning, we see that some samples decrease their angle with their class direction but the other set of samples increase the angle.
%In Fig.~\ref{fig:use_case_7_3}), two local geometric views show the positive and negative impact. 
%Through the use of ``metric difference selection" control (see Fig.\ref{fig:local_analysis_pipe_line}\textcircled{\small{4}}(a)), we can isolate samples with reduced \emph{angle} metric during the pruning process, which indicates increased performance. 
%\update{A quantification study about the }

%to incorporate class prediction uncertainty of individual samples for pruning method evaluation.
%A potential usability of these information is using these information .

%\BK{What are the implications of this analysis? Why is this interesting? Are we saying accuracy alone does not characterize the actual behavior of the models? Let us discuss this.}

%To better understand the details of geometric changes after magnitude and MPTs pruning, we take a closer look through the local geometric plots in Fig.~\ref{fig:use_case_7_2_2}. 
%The top five plots show the geometric changes of plane samples with different fraction of weight pruned using magnitude pruning. 
%From the visualization, we can see that 10\% weight pruning seems not to affect most of the samples' geometry metrics. 
%With 30\% weights pruned, we can see a notable shift in samples' geometry metrics, as indicated by the obvious trajectories in the plots. With 50\% and 70\% weights pruned,the geometric structure of samples have significant change and the predicted label of some samples are flipped. 
%Without retraining, straight forward magnitude pruning only shifts the geometric metric distribution in the negative performance direction (increase \emph{angle}, decrease \emph{length} and \emph{margin}).
%The bottom five local geometric visualization in Fig.~\ref{fig:use_case_7_2_2} show the geometry metrics changes under different pruning ratio using MPT approach. 
%The pruning operation will have positive impact until the percentage of the pruning reach a certain threshold.
%After this threshold, further pruning only cause negative impact on model's performance.

%\BK{This should be rephrased in a way that shows MPT is surprisingly better and out tool highlights something that is not trivially known from accuracy numbers. Maybe explicitly say this in next line.}


%\begin{figure}[t]
%\centering
%    \includegraphics[width=\linewidth]{images/7_use_case_5.pdf}
   
%    \vspace{-3mm}
%    \caption{Magnitude pruning will decrease the geometric features margin, \emph{length} and increase the \emph{angle}. MPTs continue to increase the \emph{margin}, \emph{length} but decrease the \emph{angle}. This trend stops when more than 90\% of weights are pruned.}
%\label{fig:use_case_7_2_2}
%\vspace{-4mm}
%\end{figure}

%Overall, pruning approaches can have a drastically different impacts on a model's latent spaces' geometric structure even if the final pruned models have a similar prediction accuracy.
%In this case, the first order Taylor pruning method does not significantly transforms the geometric structure but amplifies the ambiguity that exists in the original dense model.
%However, random pruning and the magnitude pruning not only amplify the ambiguity in the original model but also changes the geometric structure which causes new mistakes that does not exist in the original dense model.
%The models generated by MPT approach demonstrate more stable latent space structure than rest of the models and the method may be able to refine the geometric feature of the well trained model. 


%{\BK{Let us rephrase to highlight this implication.}}

%here we discuss the difference between pruning techniques and their impact over the model's inner state feature
%\begin{itemize}
%    \item regular weight training and spare model training construct similar geometric feature, but their geometric scale in these two model are significantly difference.
%    \item During the analysis, the biprop pruning can be considered as pruning and training while the regular pruning seems decrease the geometric representation.
    
%\end{itemize}



%\begin{figure}[t]
%\centering
%    \includegraphics[width=\linewidth]{images/7_use_case_3.pdf}
   
%    \vspace{-3mm}
%    \caption{Pruning approaches on the well-trained model will reshape samples' latent representation. The new feature representations can have a distinct geometric representation that causes different prediction confusion. This information is a valuable reference for constructing better feature representation with approaches such model assemble.}
%\label{fig:use_case_7_1}
%\vspace{-2mm}
%\end{figure}





